Which One? Leveraging Context Between Objects and Multiple Views for Language Grounding

When connecting objects and their language referents in an embodied 3D environment, it is important to note that: (1) an object can be better characterized by leveraging comparative information between itself and other objects, and (2) an object's appearance can vary with camera position. As such, we present the Multi-view Approach to Grounding in Context (MAGiC), which selects an object referent based on language that distinguishes between two similar objects. By pragmatically reasoning over both objects and across multiple views of those objects, MAGiC improves over the state-of-the-art model on the SNARE object reference task with a relative error reduction of 12.9\% (representing an absolute improvement of 2.7\%). Ablation studies show that reasoning jointly over object referent candidates and multiple views of each object both contribute to improved accuracy. Code: https://github.com/rcorona/magic_snare/

==> Tables/table1_sota.tex <==
\definecolor{Gray}{gray}{0.9}

\newcommand*{\belowrulesepcolor}[1]{% 
  \noalign{% 
    \kern-\belowrulesep 
    \begingroup 
      \color{#1}% 
      \hrule height\belowrulesep 
    \endgroup 
  }%
} 
\newcommand*{\aboverulesepcolor}[1]{% 
  \noalign{% 
    \begingroup 
      \color{#1}% 
      \hrule height\aboverulesep 
    \endgroup 
    \kern-\aboverulesep 
  }%
} 


\begin{table*}[t]
\centering
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
% \begin{tabular}{@{}lllllll@{}}
% \begin{tabular}{lll>{\columncolor[HTML]{c0c0c0}}llll}
\begin{tabular}{l
>{\columncolor{Gray}}r 
>{\columncolor{Gray}}r 
>{\columncolor{Gray}}r
    rrr} 
    & \multicolumn{3}{c}{\textbf{VALIDATION ACC.}} & \multicolumn{3}{c}{\textbf{TEST ACC.}}             \\
Model   & \multicolumn{1}{l}{\cellcolor{Gray}Visual}      & \multicolumn{1}{l}{\cellcolor{Gray}Blind}       & \multicolumn{1}{l}{\cellcolor{Gray}{All}}         & \multicolumn{1}{l}{Visual}        & \multicolumn{1}{l}{Blind}         & \multicolumn{1}{l}{All} \\
\toprule
Human (U)& $94.0\phantom{ (0.0)}$       & $90.6\phantom{ (0.0)}$         & $92.3\phantom{ (0.0)}$         & $93.4\phantom{ (0.0)}$           & $88.9\phantom{ (0.0)}$           & $91.2\phantom{ (0.0)}$           \\ \hline
ViLBERT & $89.5\phantom{ (0.0)}$        & $76.6\phantom{ (0.0)}$         & $83.1\phantom{ (0.0)}$         & $80.2\phantom{ (0.0)}$           & $73.0\phantom{ (0.0)}$           & $76.6\phantom{ (0.0)}$           \\
MATCH   & $89.2 (0.9)$  & $75.2 (0.7)$  & $82.2 (0.4)$  & $83.9 (0.5)$    & $68.7 (0.9)$    & $76.5 (0.5)$    \\
LAGOR   & $89.8 (0.4)$  & $75.3 (0.7)$  & $82.6 (0.4)$  & $84.3 (0.4)$    & $69.4 (0.5)$    & $77.0 (0.5)$    \\
VLG     & $91.2 (0.4)$  & $78.4 (0.7)$  & $84.9 (0.4)$  & $86.0\phantom{ (0.0)}$           & $71.7\phantom{ (0.0)}$           & $79.0\phantom{ (0.0)}$           \\ 
{\model}    & $\pmb{92.1 (0.4)}$  & $\pmb{81.3 (0.9)}$  & $\pmb{86.8 (0.5)}$  & $\pmb{87.7\phantom{ (0.0)}}$ & $\pmb{75.4\phantom{ (0.0)}}$ & $\pmb{81.7\phantom{ (0.0)}}$ \\ \bottomrule
\end{tabular}
\caption{\textbf{SNARE Benchmark Performance.} Mean accuracy $\pm$ standard deviation over 10 seeds. We find that {\model} outperforms all other models on SNARE. We find that our model is statistically significantly better than VLG, the previous state-of-the-art approach, under a Welch's unpaired two-tailed t-test with a $p<0.001$. 
% LOCKET* is a leaderboard submission to SNARE but does not have an associated paper or code at the time of writing, so the validation results are blank.
}
\label{tab:benchmarks}
\end{table*}

==> sections/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}


%Language Grounding and motivating 3D
%\textit{Language grounding} refers to the open problem of learning mappings between natural language and its corresponding representation in various domains, often encompassing visual representations~\cite{Harnad_1990}. In particular, grounded language is enriched with context from action and perception which allows for deeper semantic understanding \cite{bisk_experience_2020}. Such context is crucial for effective reasoning about natural language in domains such as vision and robotics \cite{tellex2020robots}.

%Grounding language to visual object representations is central to this kind of research. However, mapping language to 2D image representations lacks alignment with the 3D world that humans and other embodied agents interact in. While this misalignment may have minimal impact on simpler tasks like 2D object detection \cite{sadhu_zero-shot_2019}, real-world scenarios involving robot identification or grasping require leveraging various language descriptions that encompass attributes such as color, shape, and size \cite{xu_joint_2023, huang_language_2022, shridhar_alfred_2020}. Therefore, a 3D understanding of the target object would greatly benefit the robot.


% Explanation of the pragmatics approach for leveraging context intrinsic to the task

%One way to ground language in a 3D context is to consider \textit{multiple views} of an object. A collection of views provides richer information than a single 2D image for an agent to reason about. Many objects possess distinguishing features that may be overlooked in 2D. For instance, when searching for "thick" book with a "black" cover, relying solely on grounded language descriptions can be unreliable if the agent is viewing the object from a particularly inconvenient angle. In such cases, a multi-view 3D representation facilitates goal-oriented language grounding, which is particularly advantageous for object identification.

%In language grounding, it is also important to consider pragmatics, which involves leveraging contextual information from the visual and embodied world to enhance language understanding  \cite{fried_pragmatics_2022}. For example, when tasked with "the coffee mug with a thin handle" and there are two mugs with handles, the agent must reason about \textit{both} objects concurrently to comparatively decide which mug has a relatively thinner handle. In essence, the agent is using context conferred upon it by viewing both mugs to better perform at the task given the language description. In our work, we focus on grounding language to object representations using both comparative object context and multi-view context.

%Problem description with as little jargon as possible (just language grounding definition)
When an agent is asked to find the object with a ``thin handle" between two similar objects, it must contextually reason about the object with the relatively thinner handle. 
Rich context inherent in such grounded natural language descriptions can be useful for reasoning about objects in domains such as vision and robotics \cite{tellex2020robots, krishna2017visual, lu_vilbert_2019, li_grounded_2022, desai_virtex_2021}. 
% This use of context falls under the area of pragmatics, where the agent must reason about an alternative object so that the descriptor of a ``thin handle" is made more informative by comparison. 

%This use of context falls under the area of pragmatics, where contextual information can make natural language more informative. If the agent were to reason about the two objects separately, the descriptor of the ``thin handle" for each individual object is less informative than if the agent were to reason about both objects. In considering \textit{both} objects, the descriptor  ``thin handle" is made more contextually useful by comparison of both objects' distinctive features. 
\textit{Language grounding} refers to the task of learning mappings between natural language and its corresponding representation in various domains, in this case, a visual representation~\cite{Harnad_1990}. 
Models for identifying referent objects from language generally consider objects in isolation when scoring their compatibility with the referring expression~\cite{thomason_language_2021,corona_voxel-informed_2022}; however, there are cases where an agent must ground language based on the context of multiple similar objects.
Additionally, an agent with multiple views of an object is afforded further context for language grounding.
In the case of grounding the language description ``thin handle", the handle may be occluded in some viewpoints; thus, the agent must reason about the 3D shape of the mug to understand what denotes a ``thin handle". 

\input{figs/fig1_high-level_model}


% Rewrite of the first few paragraphs:
%Problem Domain
% \textit{Language grounding} refers to the open problem of learning mappings between natural language and its corresponding representation in various domains, often encompassing visual representations~\cite{Harnad_1990}. In particular, grounded language is enriched with context from action and perception which allows for deeper semantic understanding \cite{bisk_experience_2020}. Such context in natural language can be crucial in domains such as vision and robotics \cite{tellex2020robots, krishna2017visual, lu_vilbert_2019, li_grounded_2022, desai_virtex_2021}.

% Thus, object detection is one area that can benefit from the utilization of language-grounding techniques, leveraging the descriptive qualities of natural language to aid in visually identifying the referent object. In particular, our work deals with grounding language descriptors for the purpose of 3D object identification, an essential element of perceptual reasoning for embodied agents operating in the real world.

%Describing our work
We propose {\model}, a transformer-based model for 3D language grounding in object reference games.
Our model demonstrates the effectiveness of considering contextual information and reasoning over multiple objects and their views.
% The model is evaluated on the \textbf{S}hape\textbf{N}et \textbf{A}nnotated with \textbf{R}eferring \textbf{E}xpressions (SNARE) benchmark~\cite{thomason_language_2021}, an object reference task where an agent grounds natural language descriptions to household objects. 
The model is evaluated on the \textbf{S}hape\textbf{N}et \textbf{A}nnotated with \textbf{R}eferring \textbf{E}xpressions (SNARE) benchmark~\cite{thomason_language_2021}, an object referent identification from language task.
{\model} achieves improvements in language grounding accuracy compared to the previous state-of-the-art (SoTA) approach \cite{corona_voxel-informed_2022}, which does not utilize context and relies on a pre-trained 3D-voxel reconstruction model. 
Specifically, {\model} outperforms the previous SOTA by 2.7\% in overall accuracy and a 3.7\% improvement in grounding accuracy for shape-based language descriptions.

%Previous Methods in related areas

% language grounding between images exists. doesn't use context (RSA-like papers with non-contextual listeners)
% language grounding for 3d scene objects exist. their objects are all very different.
% ours requires more nuanced understanding of language
% none of these consider context. we do.


%Specifying the scope of our research
Language grounding to objects in 2D images is a commonly explored area of work \cite{sadhu_zero-shot_2019, yu_modeling_2016, plummer_flickr30k_2016, wang_improving_2021}. 
Past research has also investigated language grounding for the purpose of object localization in 3D scenes \cite{huang_multi-view_2022, liu2021referitinrgbd}. 

We distinguish our work from past research in two key ways. 
First, the task of language grounding for 3D object reference games is more granular than 3D scene understanding or object localization in 3D scenes.
In this task, an agent must identify a specific object based on a language description given a choice between it and a similar distractor, e.g. choosing one of two chairs given an object description as shown in Figure~\ref{fig:overview}. 
The task can present itself as a common scenario to embodied agents operating in real-world environments and requires a more nuanced understanding of the language for disambiguation between similar objects. 
Secondly, our \textit{pragmatically-informed} method leverages visual context to enhance language grounding \cite{potts_157pragmatics_2022,fried_pragmatics_2022}, something previous methods do not make use of. 
More concretely, our model uses context from reasoning over (i) objects and language concurrently as well as reasoning over (ii) multiple views of the objects to better perform the task of object disambiguation from a language description.

%How we are better than previous work/SOTA
Our key contributions include:
\begin{itemize}
    \itemsep0pt
    \item A novel method inspired by pragmatics that leverages multiple-object context for grounding language descriptions to object representations.
    \item {\model}---the first 3D-object, language-grounding model on the SNARE benchmark that \textit{explicitly} reasons over multiple 2D-image views of an object rather than aggregating them.
    \item {\model}'s \textbf{statistically significant SOTA performance on the validation set of the SNARE benchmark}, which leads to an absolute improvement of 2.7\% accuracy on all categories compared to the previous SOTA on the test set. \textbf{NOTE double check statistical significance}
\end{itemize}



==> sections/1_introduction_v2.tex <==
\section{Introduction}\label{sec:introduction}
%start broad: In 3D robotic tasks, A + B


%Problem description with as little jargon as possible (just language grounding definition)
When a model is asked to find the object with a ``thin handle" between two mugs, it must contextually reason about the object with the \textit{relatively thinner} handle. 
Relative pragmatic \cite{potts_157pragmatics_2022, fried_pragmatics_2022} context in grounded natural language descriptions is useful for reasoning about objects in vision and robotics~\cite{tellex2020robots, krishna2017visual, lu_vilbert_2019, li_grounded_2022, desai_virtex_2021}. 


\input{figs/fig1_high-level_model}


\textit{Language grounding} aims to connect natural language about the world to corresponding machine representations of the world~\cite{Harnad_1990}. 
Some models score referring expression compatibility with visual observations of an object in isolation~\cite{thomason_language_2021,corona_voxel-informed_2022}, while broader methods for aligning vision and language representations often consider only static images of objects and scenes~\cite{radford_learning_2021,kim2021vilt}.
However, language meant to distinguish objects of the same category can contain comparative information to identify the correct referent~\cite{grice1975logic}, and multiple viewpoints of objects may be needed.
For example, mug handles are occluded in certain viewpoints, and referring to a mug as one with a ``thin handle" implies ``a handle thinner than those of the other mugs at play.''




%Describing our work
To address this gap, we introduce {\modelfull} ({\model}).
\model\ jointly reasons over candidate referent objects, each considered from multiple possible vantage points (Figure~\ref{fig:overview}). 
% This 3D object reference task is more granular than 3D scene understanding or object localization in 3D scenes, which often focus on distinguishing and localizing objects of different, i.e. visually distinct, classes.
% Previous work for object reference tasks considers only a single object at a time, thus past methods are unable to contextually reason about the differences between objects, a skill that is essential for language grounding of similar objects.
% Existing work on object reference tasks considers only one object at a time, which limits the ability to reason about the relative differences between objects. 
% However, this contextual reasoning is crucial for successfully grounding language descriptions of similar objects.
% Thus we propose a {\modelfull} ({\model}), a transformer-based model that uses context from reasoning over (i) the relative references between the object and language concurrently as well as reasoning over (ii) multiple views of the objects to better perform the task of object disambiguation from a language description.
We evaluate \model\ via the \textbf{S}hape\textbf{N}et \textbf{A}nnotated with \textbf{R}eferring \textbf{E}xpressions (SNARE) benchmark~\cite{thomason_language_2021}.
In SNARE, candidate objects are always of the same high-level category, such as \textit{chair} or \textit{mug}, and language references uniquely identify one target referent object in contrast to the distractor object of the same category.
Embodied agents operating in real-world environments analogously need to disambiguate between similar objects, such as mugs in a kitchen, parts on a conveyor belt, or rocks on the seafloor.
By reasoning about both objects and their views, \model\ improves accuracy over existing models by 2.7\%.
Our contributions include:
\begin{itemize}[noitemsep,nosep]
    \item {\model}, a transformer-based model that reasons over multiple 2D-image views of 3D objects and implicitly considers the relative differences between objects;
    \item state-of-the-art SNARE accuracy\footnote{\href{https://github.com/snaredataset/snare\#leaderboard}{https://github.com/snaredataset/snare\#leaderboard}}
    \item ablation studies suggesting that both multi-object and multi-view inputs are needed for the {\model} accuracy gains and
    \item analysis suggesting {\model} outperforms previous methods as all are restricted to fewer object viewpoints.
\end{itemize}

% In short, we introduce {\modelfull} ({\model}), the first 3D-object, language grounding model on the SNARE benchmark that \textit{explicitly} reasons over multiple objects and their views. 

==> sections/2_related_work.tex <==
\section{Background and Related Work}\label{sec:related_work}

Our work aims to address important questions in vision, language, and robotics. 
As embodied agents increasingly operate in shared environments with humans, it becomes crucial for them to understand the relationships between natural language expressions and the objects they refer to.
However, achieving this level of understanding requires agents to go beyond local object perception and consider similar objects in a broader global context.
Thus, the research areas of object identification, language grounding, and pragmatics are essential for enabling agents to interact with objects in real-world settings in context.

\subsection{Object Identification.} 

Image and object classification are some of the simplest examples of perceptual reasoning for an agent or model to accomplish. 
Robust performance on these types of tasks has been established with CNN and ResNet architectures \cite{simonyan_very_2015, he_deep_2015, huang_densely_2017}. 
These architectures have demonstrated robust performance in classification tasks.
For more fine-grained tasks such as image segmentation and object identification, there has been significant progress with the advent of architectures like R-CNNs and transformers \cite{girshick_rich_2014, carion_end--end_2020}. 


Existing methods broadly in the area of 3D object identification have approached the problem in a variety of ways. 
The most common method originated from the work on PointNet \cite{qi_pointnet_2017}, which promoted a rise in research leveraging point clouds for 3D object detection \cite{qi2018frustum, zhou2018voxelnet}. 
Another similar area of work focuses generally on 3D scene understanding or more specifically, on localizing objects in a 3D scene \cite{zhang2017deepcontext, huang2018cooperative, huang_multi-view_2022}. 
Distinct from this previous work, our research focuses on the problem of identifying the referent of a language descriptor when given both the 3D referent object and a similar distractor object. 
% To facilitate this, we make use of a transformer-based architecture.
% We explore the usage of a transformer architecture for this purpose.

Transformers have proven to be effective in handling both language and vision data, leading to significant improvements in perceptual tasks \cite{lu_vilbert_2019, xu_joint_2023, desai_virtex_2021}. 
They also yield propitious results in tasks where language plays a central role, such as image captioning and visual question-answering \cite{agrawal_vqa_2016, wang_end--end_2022, xu_multimodal_2023}.
Thus, we leverage a transformer-based architecture, a promising choice for the task of disambiguating a 3D object given a natural language description.
% These encouraging outcomes motivate further research in this domain.

\subsection{3D Language Grounding.} 

In the domain of grounding language to visual representations, significant progress has been made in 2D settings \cite{sadhu_zero-shot_2019, yu_modeling_2016, plummer_flickr30k_2016, wang_improving_2021}.
However, 2D image data often intrinsically incorporates many perceptual assumptions that limit its applicability in the real world. 
The standard paradigm of using ideal images with important physical features of objects in full view is not emblematic of realistic situations embodied agents will be working in.
For instance, consider the scenario where an embodied agent needs to ground a natural language expression referring to the shape of a mug's handle.
Grounding such a description becomes more challenging when relying on a static, 2D image where the entire handle is simply rotated out of view.

To address these limitations, the field of 3D language grounding has emerged as a promising direction.
Generally, previous work involved mapping language expressions to various 3D object and scene representations, such as meshes \cite{cohen_grounding_2019}, point cloud networks \cite{nichol_point-e_2022, guo_deep_2020, achlioptas_shapeglot_2019, koo2022partglot}, light field networks \cite{sitzmann_light_2022}, neural radiance fields \cite{yu_pixelnerf_2021}, and voxels \cite{corona_voxel-informed_2022}. 
These explicit 3D representations are useful in alleviating the limitations of 2D images. 
However, while yielding these benefits, these 3D representations are, in essence, an additional assumption of the type of data that will be available or need to be generated for a task. 
Thus, our model exploits multiple 2D-image views of objects to take advantage of the 3D information without the need for explicit 3D representations.
% These representations are useful in mitigating the limitations inherent in 2D images, and their application to our work will be discussed later in the paper.
% Beyond object detection, language grounding in 3D has been advantageous in more granular tasks such as path-planning and instruction-following for embodied agents in real-world environments \cite{shridhar_alfred_2020, zhang_hierarchical_2021, huang_language_2022,blukis2022persistent}.


Multiple datasets have been developed to address the object reference task for 3D language grounding.
ShapeGlot \cite{achlioptas_shapeglot_2019} considers a dataset of chairs and lamps and trains a model that distinguishes a target object from a set of 2 distractor objects using shape-based language descriptions.
PartGlot \cite{koo2022partglot} extends the use of this reference task to learn point cloud part-segmentation implicitly using a transformer-based cross-attention module.
In contrast, SNARE \cite{thomason_language_2021} utilizes the ShapeNetSem dataset, which includes 262 object categories, allowing for the evaluation of language grounding across diverse object classes. 
ChangeIt3D \cite{achlioptas2022changeIt3D} introduces its own dataset comprising 29 object classes, with a focus on learning grounded point cloud representations for 3D shape editing. 
In our work, we concentrate on the SNARE dataset due to its large number of object classes, enabling us to demonstrate the generalizability of our approach.


%\textbf{Potentially remove this because it is covered later, or combine it with the later description}To serve as an evaluation for our work, we test our model on the SNARE benchmark. The SNARE dataset is an object-reference task that consists of a subset of 7,897 objects from the ACRONYM grasping dataset as well as multiple natural language descriptions for each referent object \cite{thomason_language_2021, eppner_acronym_2020}. The task presents a model with two objects---each as a set of 8 image views---as well as a referring expression that corresponds to one of the objects. The goal of the model is to correctly classify the referent object that corresponds to the referring expression. As opposed to standard 3D language grounding tasks that localize distinct objects in a 3D scene \cite{huang_multi-view_2022}, SNARE's objects for a given instance are adversarially selected to be similar. By evaluating the performance of our model on similar objects across different categories, we can assess our model's ability to generalize in different contexts.}

\subsection{Pragmatics}

Our research gathers inspiration from \textit{pragmatics} in linguistics. 
In the pragmatics paradigm, language is not simply a series of utterances, but rather, it is a holistic integration of both semantic meaning and broader contextual information \cite{potts_157pragmatics_2022}. 
Indeed, one of the most noteworthy insights of pragmatics is the fact that language descriptions are context-dependent.
In order to account for this context dependency in conversation, it is necessary to establish \textit{common ground}, which is the set of fundamental base principles and assumptions all actors in a pragmatic model are subject to \cite{potts_157pragmatics_2022, fried_pragmatics_2022, bao_learning_2022}. 

One important goal of linguistics is thus to incorporate common ground into speaker-listener models of conversation such as the Rational Speech Acts (RSA) model, a recursive process between a probabilistically-modeled speaker and listener \cite{monroe_learning_nodate}. This can involve specifying social and communicative norms, temporal context, task goals, and common knowledge that can be elicited from multiple modalities \cite{fried_pragmatics_2022, bisk_experience_2020}. At a high level, the object reference task problem mirrors the RSA formulation. One can view the SNARE benchmark as a static speaker while {\model} acts as the listener that tries to achieve a contextual understanding of the speaker.
% Research in multi-agent settings is a great example of a field where the incorporation of context, whether in the model itself or the "world representation", has become a common facet of emerging research \cite{lowe_multi-agent_2017, rogers_tracing_2023, park_generative_2023, kang_recommendation_2019, shridhar2022peract}.

In the applications of developing grounded language and embodied agents in real-world environments, establishing a common-ground context is crucial for mutual perceptual understanding among agents.
This can be achieved through the use of visual information and interaction with the environment. 
For example, previous work has focused on incorporating visual context to generate image captions that are "pragmatically informative."
This means that the generated captions not only accurately describe the image but also effectively distinguish it from other similar images \cite{cohn-gordon_pragmatically_2018}. 
Similarly, our work is unique from past SOTA in the field of language grounding for 3D object reference tasks in that it employs pragmatic reasoning to be able to distinguish similar objects based on a descriptive caption. 
% Additionally, there have been pragmatic methods explored that adjust the content of language expressions between a speaker and listener agent to address the inherent knowledge disparity between the two \cite{bao_learning_2022}.
% These approaches highlight the importance of considering pragmatics in language grounding in real-world scenarios.
